An Energy-Aware On-Demand Routing Protocol for Ad-Hoc Wireless Networks

An ad-hoc wireless network is a collection of nodes that come together to dynamically create a network, with no fixed infrastructure or centralized administration. An ad-hoc network is characterized by energy constrained nodes, bandwidth constrained links and dynamic topology. With the growing use of wireless networks (including ad-hoc networks) for real-time applications, such as voice, video, and real-time data, the need for Quality of Service (QoS) guarantees in terms of delay, bandwidth, and packet loss is becoming increasingly important. Providing QoS in ad-hoc networks is a challenging task because of dynamic nature of network topology and imprecise state information. Hence, it is important to have a dynamic routing protocol with fast re-routing capability, which also provides stable route during the life-time of the flows. In this thesis, we have proposed a novel, energy aware, stable routing protocol named, Stability-based QoS-capable Ad-hoc On-demand Distance Vector (SQ-AODV), which is an enhancement of the well-known Ad-hoc On-demand Distance Vector (AODV) routing protocol for ad-hoc wireless networks. SQ-AODV utilizes a cross-layer design approach in which information about the residual energy of a node is used for route selection and maintenance. An important feature of SQ-AODV protocol is that it uses only local information and requires no additional communication or co-operation between the network nodes. SQ-AODV possesses a make-before-break re-routing capability that enables near-zero packet drops and is compatible with the basic AODV data formats and operation, making it easy to adopt in ad-hoc networks.

==> sq-aodv-in-ns-2.tex <==
\cleardoublepage
\phantomsection
\addcontentsline{toc}{chapter}{Appendix}
\appendix
\chapter{Introduction to NS-2}
\label{intro-ns-2}
NS-2 is an object-oriented, discrete event driven network simulator written in C++ and OTcl (Object-oriented Tool command language). NS-2 provides substantial support for simulating wired and wireless networks with network protocols such as TCP and UDP. NS-2 has support for, traffic source behavior such as FTP, Web, CBR and VBR, router queue management mechanism such as Drop Tail, RED and CBQ, standard routing protocols and Link layer protocols for both wired and wireless networks.

Although NS-2 is very easy to use once you get to know it, but is quite difficult for a beginners. To get a feel of what is NS-2, a beginner is recommended to exercise some of the examples given in~\cite{NS-BY-EX}. One can find a more detailed documentation of NS-2 in~\cite{NS-DOC}, which is written with the depth of a skilled user.

NS-2 is written in both C++ and OTcl languages, with data path using C++ and control path using OTcl. In order to reduce the packet and event processing time, the event scheduler and the basic network component objects are written and compiled using C++. These compiled objects are made available to OTcl interpreter through OTcl linkage as shown in Fig.~\ref{fig41}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
	\centering
	\includegraphics[scale = 0.45]{OTcl-and-c++-linkage-in-NS-2.eps}
	\caption{C++ and OTcl Linkage in NS-2}
	\label{fig41}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The OTcl linkage creates a matching OTcl object for each of the C++ objects. Thus giving the control of the C++ objects to OTcl. There are objects in C++ that do not need OTcl control, these objects are not in OTcl space. Similarly there are objects that are entirely implemented in OTcl and are not in C++ space. Thus, there is a matching OTcl object hierarchy very similar to that of C++. We now give a very brief explanation as how NS works.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
	\centering
	\includegraphics[scale = 0.45]{Simplified-users-view-of-NS-2.eps}
	\caption{Simplified User's View of NS-2}
	\label{fig42}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As shown in Fig.~\ref{fig42}, NS-2 is Object-oriented Tcl (OTcl) script interpreter that has a simulation event scheduler and network component object libraries, and network setup helping module libraries. The procedure for simulating a network scenario using NS-2 is as follows: User has to write a program using OTcl script language. This program basically initiates an event scheduler , sets up a network topology using network component objects and helping modules, and tell the traffic sources when to start and stop the transmission of packets through event scheduler. This OTcl script is executed by NS-2 to generate the trace of events. The the event scheduler will keep track of simulation time and dumps all the events of the event queue scheduled at the current time into an output file to generate the trace file output. Thus generated trace file is further processed by user written scripts to analyze the simulation results. Alternatively, the simulation results can also be visualized using Network AniMater (NAM) 

\chapter{Implementation of SQ-AODV in NS-2}
\label{sq-aodv-details-in-ns-2}
In this chapter we provide implementation details of SQ-AODV in Network Simulator Version-2~\cite{NS-2} (NS-2). Since we have modified AODV routing protocol, we explain the implementation of AODV, and the modifications made to make it SQ-AODV. We first, give a brief introduction to NS-2, then give the implementation details of SQ-AODV. 

\subsection{Route Discovery in SQ-AODV}

When a source node wants to communicate with a destination, the application layer generates the data packets and send them to the network layer. When we use AODV as routing protocol, the packet arrived at the network layer (Routing layer) will be received by AODV::recv(Packet *p, Handler *h). The basic operation of the recv function is depicted in Fig.~\ref{fig43}. Now if the packet is an AODV type then, it is further processed by AODV::recvAODV(Packet *p) and its operation is depicted in Fig..~\ref{fig46}. If the packet is a data packet and the current node is the originator then, update the Time To Live (TTL) field of the IP header as required for a broadcast or unicast packet. If the packet is a broadcast packet then forward the packet using AODV::forward(aodv$\_$rt$\_$entry* 0, Packet *p, double delay), else if the packet is an unicast packet then, it is further processed by AODV::rt$\_$resolve(Packet *p).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
	\centering
	\includegraphics[scale = 0.7]{recv.eps}
	\caption{Flow-chart of AODV::recv() Function}
	\label{fig43}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
	\centering
	\includegraphics[scale = 0.7]{rt_resolve.eps}
	\caption{Flow-chart of AODV::rt$\_$resolve() Function}
	\label{fig44}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
	\centering
	\includegraphics[scale = 0.75]{sendRequest.eps}
	\caption{Flow-chart of AODV::sendRequest() Function}
	\label{fig45}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
	\centering
	\includegraphics[scale = 0.75]{recvAODV.eps}
	\caption{Flow-chart of AODV::recvAODV() Function}
	\label{fig46}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The basic operation of rt$\_$resolve is depicted in Fig.~\ref{fig44}, this function is responsible for looking a suitable path if it exists for the data packets. If a path does not exist then  initiate a route discovery process. When the data packet arrives, the transmit failure callback is \textbf{SET}, this will not change during the entire life of the data packet. This information is useful in case of packet transmission failure due to link, or drop due to queue overflow. Now, if a route to the destination if it exists, is found using function rtable.rt$\_$lookup(nsaddr$\_$t dst). If the route does not exist then, add a route using function rtable.rt$\_$add(nsaddr$\_$t dst). If the current node is source of the packet and it does not have a route to the destination, it will enqueue the packet and start a route discovery by initializing a request using AODV::sendRequest(nsaddr$\_$t dst) function. If the node is not a source node and a route exist but is IN$\_$REPAIR state, then enqueue the packet else, if the route does not exist then initiate a recovery process by sending an error packet using the function AODV::sendError(Packet* rerr, bool false).

If a node is an originator of the data packets and does not have a route to the destination, then it initiates a route discovery by broadcasting Route Request (RREQ) packet. broadcasting of RREQ packets is done by sendRequest function and its basic operation is as depicted in Fig.~\ref{fig45}. The node first, checks whether there exist a valid route to the desired destination and is UP, second, whether the route request has timed out. If one of these two checks are satisfied then the discovery process is aborted. The node does these extra check before sending a RREQ packet. The node verifies, whether the number of retries have reached the threshold value, if it has reached, the node drops all the data packets destined for this destination and reset the retry counter and abort the discovery process. Finally node updates the TTL and timeout entries of routing table and create a RREQ packet and broadcast it to its neighbors.

A RREQ packet, once received by the recv function of a node, is further processed by recvAODV function. The basic operation of recvAODV is as depicted in Fig.~\ref{fig46}. In this function the packet is sent to either one of these functions, AODV::recvRequest(Packet *p) or AODV::recvReply(Packet *p) or AODV::recvError(Packet *p)
or AODV::recvHel-\\lo(Packet *p), depending on whether the packet is, request or reply or error or hello respectively. Thus the RREQ packet reaches the recvRequest function of a node for further processing. The operation of the recvRequest function is depicted in Figs.~\ref{fig47} and~\ref{fig47_A}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
	\centering
	\includegraphics[scale = 0.75]{recvRequest.eps}
	\caption{Flow-chart of AODV::recvRequest() Function}
	\label{fig47}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
	\centering
	\includegraphics[scale = 0.75]{recvRequest_A.eps}
	\caption{Flow-chart of AODV::recvRequest() Function}
	\label{fig47_A}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
	\centering
	\includegraphics[scale = 0.75]{sendReply.eps}
	\caption{Flow-chart of AODV::sendReply() Function}
	\label{fig48}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
	\centering
	\includegraphics[scale = 0.75]{recvReply.eps}
	\caption{Flow-chart of AODV::recvReply() Function}
	\label{fig49}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The recvRequest function aborts the processing of RREQ packet under two conditions, one, node itself is the source of the RREQ packet, two, the broadcast id of RREQ already exists in the node cache. If the broadcast id does not exist in the cache of the node, the node caches it. The node checks for the existence of a valid route to the source (reverse route), if it exists it updates the routing table, else adds one. The node also check if any packets in the queue get benefited out of the reverse route, if yes, all these packets are forwarded using this route. Now once the reverse route is setup, node checks for the existence of a valid route to the destination. If the node is a destination node, it sends a Route Reply (RREP) packet to the source using reverse route. If the node is an intermediate node and the existing route is fresh enough, then it inserts, a previous hop and a next hop as the precursor for reverse and forward route respectively, then sends a RREP packet to the source. If the existing route in the intermediate node is not fresh enough, the RREQ packet is re-broadcasted to all its neighbors. Thus a RREQ packet once reached to the destination will definitely make the destination to send a RREP packet. The reply packet is sent using the function AODV::sendReply(nsaddr$\_$t ipdst, u$\_$int32$\_$t hop$\_$count, nsaddr$\_$t rpdst, u$\_$int32$\_$t rpseq, u$\_$int32$\_$t lifetime, double  timestamp) and  its operation is depicted in Fig.~\ref{fig48}.

The sendReply function first find a route to the source of data packets (reverse route). Then it creates a RREP packet and forwards it using the reverse route. This RREP packet is received by the recv function of a node, the recv function sends it to recvAODV for further processing. The recvAODV function further sends this RREP packet to AODV::recvReply() function for further processing. The operation of the recvReply function is depicted in Fig.~\ref{fig49}.

The recvReply first finds the existence of a valid route to the destination (forward route), if it does not exist, adds one. If the forward route exist it updates the routing table. now if the RREP packet is at the intermediate node, it uses the reverse route to forward the RREP packet further towards the source of the data packets and adds the previous hop as a precursor for the reverse path. If the node is the source node, it forwards all the packets awaiting for this destination.

This completes the Route Discovery process in AODV routing protocol, we now see the route maintenance.

\subsection{Route Maintenance in SQ-AODV}
AODV has capabilities of both proactive and reactive route maintenance. The proactive maintenance is by periodic hello messages, in this method every node in the network broadcast hello messages to its neighbors every one second. If the reactive maintenance is enabled then proactive maintenance (NeighborTimer and HelloTimer) is disabled. Reactive maintenance is done by sending ERROR packets to the sources when ever the link layer detects a link breakage.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
	\centering
	\includegraphics[scale = 0.75]{rt_ll_failed.eps}
	\caption{Flow-chart of AODV::rt$\_$ll$\_$failed() Function}
	\label{fig410}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
	\centering
	\includegraphics[scale = 0.75]{log_link_broke.eps}
	\caption{Flow-chart of AODV::log$\_$link$\_$broke() Function}
	\label{fig411}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
	\centering
	\includegraphics[scale = 0.75]{log_link_delete.eps}
	\caption{Flow-chart of AODV::log$\_$link$\_$delete() Function}
	\label{fig412}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Every data packet passes through the rt$\_$resolve function as in Fig.~\ref{fig44} in which rt$\_$failed$\_$callback is \textbf{SET}. Using this information link layer calls the function AODV::rt$\_$l-\\l$\_$failed(Packet *p), when a packet drop due to link breakage occurs. The basic operation of rt$\_$ll$\_$failed function is depicted in Fig.~\ref{fig410}. The function first checks whether the packet is a control packet or a broadcast packet, if so, it drops the packet and abort the process. If the packet is a data packet, then it first logs the packet drop with the reason for its drop using AODV::log$\_$link$\_$broke(Packet *p) function. The basic operation of the log$\_$link$\_$broke is as depicted in Fig.~\ref{fig411}.

The function further looks for a route availability to the destination of the data packet, if there is one, then drops the packet and abort the process to declare the link failure detection is false. In case of non-existence of a route, the function logs a link delete with the destination information of the link using AODV::log$\_$link$\_$delete(nsaddr$\_$t dst) function. The basic operation of the log$\_$link$\_$delete is as depicted in Fig.~\ref{fig412}. The function after loging the link delete, checks whether the dropped packet is close to the destination, if so, does a local repair using AODV::local$\_$rt$\_$repair(aodv$\_$rt$\_$entry *rt, Packet *p) function, if not drop all the packets using this route. Finally delete the unreachable neighbor from the neighbor list using the function AODV::nb$\_$delete(nsaddr$\_$t id). The operation of functions local$\_$rt$\_$repair and nb$\_$delete are dipicted in Figs.~\ref{fig413} and \ref{fig414}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
	\centering
	\includegraphics[scale = 0.75]{local_rt_repair.eps}
	\caption{Flow-chart of AODV::local$\_$rt$\_$repair() Function}
	\label{fig413}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
	\centering
	\includegraphics[scale = 0.75]{nb_delete.eps}
	\caption{Flow-chart of AODV::nb$\_$delete() Function}
	\label{fig414}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The local$\_$rt$\_$repair function first, enqueue the packet and set the status of the route as IN$\_$REPAIR. Finally initiates a route discovery by sending a RREQ packet. The nb$\_$delete function logs the link deletion information using log$\_$link$\_$delete function, then delete the unreachable node form the neighbor list. Finally initiates a link failure recovery using AODV::handle$\_$link$\_$failure(nsaddr$\_$t id) function. The basic operation of handle$\_$link$\_$failure is depicted in Fig.~\ref{fig415}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
	\centering
	\includegraphics[scale = 0.75]{handle_link_failure.eps}
	\caption{Flow-chart of AODV::handle$\_$link$\_$failure() Function}
	\label{fig415}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The function, handle$\_$link$\_$failure is responsible for sending error packets towards the source node of a route experienced the link failure. This function first finds all routes whose destination is the unreachable node. Then the status of all these routes are changed to RT$\_$DOWN along with restting the other entries to default state using AODV::rt$\_$down(aodv$\_$rt$\_$entry *rt) as depicted in Fig.~\ref{fig416}. The handle$\_$link$\_$failure function further deletes all the precursor entries of these routes whose state has been changed to RT$\_$DOWN and finally initiates a route recovery process by sending an error packet using AODV::sendError(Packet *p, bool jitter=true) function. The basic operation of sendError function is as depicted in Fig.~\ref{fig417}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
	\centering
	\includegraphics[scale = 0.75]{rt_down.eps}
	\caption{Flow-chart of AODV::rt$\_$down() Function}
	\label{fig416}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
	\centering
	\includegraphics[scale = 0.75]{sendError.eps}
	\caption{Flow-chart of AODV::sendError() Function}
	\label{fig417}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
	\centering
	\includegraphics[scale = 0.75]{recvError.eps}
	\caption{Flow-chart of AODV::recvError() Function}
	\label{fig418}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The sendError function basically creates an ERROR packet and schedule it for broadcast. This broadcasted packet is received by the AODV::recvError(Packet *p) function via recv and recvAODV functions. After receiving the ERROR packet, the recvError function first looks for a valid route availability to the unreachable destination. If a route exist but is not UP and the current node is the source of the route which we are looking for, then the function just free the ERROR packet because the source in any case start a route discovery process if the route is required. Now if the route is not UP, but it exists and the current node is an intermediate node. The node broadcast an ERROR packet using the sendError function. On the other hand if the route exists and is UP, the status of the route is changed to RT$\_$DOWN using rt$\_$down function and all the packets using this route are dropped.

Thus when the ERROR packet finally reaches all the sources which use the unreachable node as intermediate node or destination for one of their sessions will come to know about the link failure and they start a fresh route discovery process if required. This is how the proactive route maintenance in AODV works.

\subsection{Make-Before-Break Re-routing Feature of SQ-AODV}
In this section we explain the implementation level details of make-before-break feature of SQ-AODV. To implement make-before-break re-routing mechanism, we have added a timer called rcr-timer in the basic AODV code. The rcr-timer expires every 100 msec, on every expiry, the AODV::rcr() function is called. The combined operation of rcr-timer and rcr function is as depicted in Fig.~\ref{fig419}. In rcr function, a check is performed to find whether the current-energy of the current node is less than Threshold-2. If so, a Route Change Request (RCR) packet is broadcast to the 1-hop neighbors of this node.

After receiving the broadcast RCR packet, each neighbor will check whether the drained node is a destination or source or an intermediate node of a route. This check is performed for energy routing table entry and depending on whether drained node is source/destination/intermediate node for the flows of neighbors, each neighbor processes the RCR packet uniquely as depicted in Fig.~\ref{fig420}.

If the drained node is, a destination of any flow in the routing table of neighbor indicating its destination has drained and the neighboring node which received the broadcast RCR is a source of the flow, then the source node will immediately stop the traffic, on the other hand, if the neighboring node which received the broadcast RCR is an intermediate node of the flow, then this intermediate node sets the rcr-flag in the routing table and sends an unicast RCR packet towards the source of the flow.

If the node from which a broadcast RCR has come happens to be a source for any of the routes in the routing table of neighbors, then the neighboring node simply free this broadcast RCR packet.

If the node from which a broadcast RCR has come happens to be an intermediate node for any of the routes in the routing table of neighbors, and if the 1-hop neighboring node is a source of the flow, then the source broadcast a RREQ packet to initiate a route discovery process. On the other hand, if the node which received the broadcast RCR is an intermediate node of a flow, then this intermediate node sets the rcr-flag in the routing table and sends an unicast RCR packet towards the source of the flow.

In case of a route with more than one hop, an intermediate node has to unicast the RCR packet towards the source of the flow. Now, if this unicasted RCR packet has reached one more intermediate node of the flow, then this intermediate node forwards the RCR packet using the reverse route information in its routing table. On the other hand if the unicasted RCR has reached a source node of a flow, the source node will check whether the drained node is a destination or intermediate node, if the destination has drained then, the source simply stops the traffic, else if an intermediate node has drained then source initiates a route discovery process by broadcasting a RREQ packet.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
	\centering
	\includegraphics[scale = 1.12]{rcr.eps}
	\caption{Combined flow-chart of rcr-timer and rcr function}
	\label{fig419}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
	\centering
	\includegraphics[scale = 1.12]{make-before-break.eps}
	\caption{Flow-chart of make-before-break}
	\label{fig420}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
